Difficulty-Aware Simulator for Open Set Recognition

Open set recognition (OSR) assumes unknown instances appear out of the blue at the inference time. The main challenge of OSR is that the response of models for unknowns is totally unpredictable. Furthermore, the diversity of open set makes it harder since instances have different difficulty levels. Therefore, we present a novel framework, DIfficulty-Aware Simulator (DIAS), that generates fakes with diverse difficulty levels to simulate the real world. We first investigate fakes from generative adversarial network (GAN) in the classifier's viewpoint and observe that these are not severely challenging. This leads us to define the criteria for difficulty by regarding samples generated with GANs having moderate-difficulty. To produce hard-difficulty examples, we introduce Copycat, imitating the behavior of the classifier. Furthermore, moderate- and easy-difficulty samples are also yielded by our modified GAN and Copycat, respectively. As a result, DIAS outperforms state-of-the-art methods with both metrics of AUROC and F-score. Our code is available at https://github.com/wjun0830/Difficulty-Aware-Simulator.

==> _6_implementation_detail.tex <==
\vspace{-0.2cm}
\subsection{Implementation details}
% \begin{table}[]
%     \begin{tabular}{lll}
%     \hlineB{2.5}
%     % \multicolumn{1}{l|}{Layer} & \multicolumn{1}{l|}{Norm} & Activation \\ \hline
%      \multicolumn{1}{c}{Layer (stride)} &  \multicolumn{1}{c}{Norm} & \multicolumn{1}{c}{Activation} \\ \hline
%     % \multicolumn{3}{c}{Dropout}                                         \\\hline
%     3x3 Convolution (1)   & BatchNorm                 & LeakyReLU  \\%\hline
%     3x3 Convolution (1)   & BatchNorm                 & LeakyReLU  \\%\hline
%     3x3 Convolution (2)   & BatchNorm                 & LeakyReLU  \\
%     \hlineB{2.5}
%     \end{tabular}
% 	\caption{Architecture of the Convolutional Group}
% 	\label{table_convgroup}
% \end{table}
DIAS is an end-to-end framework that all components are learned from the scratch.
For the Copycat and the classifier, we use vanilla CNN~\cite{neal2018osrci}, which is composed of 9 convolution layers.
For the subgroups of convolutional layers, each group contains three 3x3 convolution layers.
% For the subgroups of convolutional layers, each group contains three 3x3 convolution layers each with the batch normalization layer\cite{ioffe2015batchnorm} and LeakyReLU activation function.
Additionally, the backbone network for the generator and the discriminator each contains 4 convolutional layers. 
Moreover, we adopt multi-batch normalization layers to process generated images from GAN separately, as we hope to prevent the problem from distribution mismatch, following \cite{chen2021arpl}.
% Note that features from the Copycat do not need multi-batch normalization layers.
Note that features from the Copycat do not need to be processed separately.
For scaling parameters, we fix both $\lambda$, and $\beta$ to 0.1.
% We also fix the $\alpha_{hard}$ and $\alpha_{easy}$ to 0.5 and 1.0.
% $\alpha_{hard}$ is further investigated in \cref{table_smoothing_ablation}.
% For hyperparameters, as we noted set ,empirically.



% To implement a copycat, we divide both copycat and classifier into subgroups of convolution layers.
% % We show the architecture of our convolutional group in \cref{table_convgroup}.
% Each subgroup contains three 3x3 convolutional layers each with the batch normalization layer\cite{ioffe2015batchnorm} and LeakyReLU activation function.
% Moreover, we adopted multi batch normalization layer to process each original image and the generated image from GAN as we hope to prevent the problem from distribution mismatch, following \cite{chen2021arpl}.
% Note that, features from the copycat do not need multi batch normalization layer.

% For all experiments, we use vanilla CNN architecture~\cite{neal2018osrci} for both the copycat and the classifier which is composed of 9 convolutional layers.
% The generator and the discriminator contains 4 convolutional layers. 
% For the hyperparameters, we set $\alpha$ $\lambda$
% % For hyperparameters, as we noted set ,empirically.

==> _7_reference.tex <==
\small
\bibliographystyle{ieee_fullname}
\bibliography{egbib}
